Spatially Selected and Dependent Random Effects for Small Area Estimation with Application to Rent Burden

Area-level models for small area estimation typically rely on areal random effects to shrink design-based direct estimates towards a model-based predictor. Incorporating the spatial dependence of the random effects into these models can further improve the estimates when there are not enough covariates to fully account for spatial dependence of the areal means. A number of recent works have investigated models that include random effects for only a subset of areas, in order to improve the precision of estimates. However, such models do not readily handle spatial dependence. In this paper, we introduce a model that accounts for spatial dependence in both the random effects as well as the latent process that selects the effects. We show how this model can significantly improve predictive accuracy via an empirical simulation study based on data from the American Community Survey, and illustrate its properties via an application to estimate county-level median rent burden.

==> latexmkrc <==
# HACK: this width seems to change with every compile, so
# latexmk runs latex too many times; ignore it
$hash_calc_ignore_pattern{'aux'} = 'statsocwidth';

# All the other default settings on Overleaf
# support for the glossaries package:
add_cus_dep('glo', 'gls', 0, 'makeglossaries');
add_cus_dep('acn', 'acr', 0, 'makeglossaries');
sub makeglossaries {
  system("makeglossaries \"$_[0]\"");
}

# support for the nomencl package:
add_cus_dep('nlo', 'nls', 0, 'makenlo2nls');
sub makenlo2nls {
  system("makeindex -s nomencl.ist -o \"$_[0].nls\" \"$_[0].nlo\"");
}

# from the documentation for V. 2.03 of asymptote:
sub asy {return system("asy \"$_[0]\"");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

# metapost rule from http://tex.stackexchange.com/questions/37134
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

==> scratch.tex <==
% The U.S. Census Bureau’s SAIPE program is the primary source of annual estimates of income and poverty statistics for all states and counties. These estimates, derived from SAE models, are used for the administration of federal programs and allocating billions of dollars of federal funds to local jurisdictions \todo{Source}.  The SAIHE program serves a similar purpose for estimating healthcare coverage across the U.S., aiding programs such as the Affordable Care Act  [2].  An SAE model is also used to implement Section 203 of the Voting Rights Act [3] \todo{Source}. Section 203 determines which local jurisdictions are required by law to provide translated voting material to their citizens, supporting the functioning of the American democratic system. 



Both 

Some recent extensions of the FH model have utilized \textit{shrinkage} in the priors for the random effects. This describes the phenomenon that many standard estimators can be improved, in terms of mean squared error, by biasing estimates towards zero\footnote{In this setting the idea is to "shrink" the random effects that are not needed to zero. Note that this is not to be confused with "shrinkage" area level models to describe how much the area-specific direct estimators is brought toward the regression based estimate. }.  One promising Bayesian solution has been proposed by Datta and Mandal (2015) using a spike-and-slab prior for the random effects. \todo{Source} Their approach uses the data to 'select' each of the random effects: shrinking some of the random effects to a point-mass at zero while the rest are modeled using an independent normal distribution. Tang, Ghosh, Ha, \& Sedransk (2018) subsequently proposed a model that is a continuous analog of the Datta-Mandal approach by using the class of Global-Local priors. \todo{Source} 



For GL model, the global parameter $\tau^2$ acts in a similar way to $p$ in the DM model which controls the shrinkage of all areas (hence the term "global"). The local parameters $\lambda_i^2$ accounts for the area-to-area differences in the random effect shrinkage. A more detailed discussion about shrinkage factors can be found in Tang et al. (2018). \todo[inline, color=green!40]{Note: Could be cut? }



A continuous analog to the DM model was introduced by Tang, Ghosh, Ha, \& Sedransk (2018) \todo{Source} using the fast-expanding class of Global-Local Shrinkage Prior for the random effects
\begin{align}
  \bb u \given \tau^2, \Lambda \sim N_n(\bb 0, \tau^2 \Lambda), 
\end{align}
where $\Lambda = \textrm{diag} \set{\lambda^2_1, \cdots, \lambda^2_n}$ and with a prior of the form $\pi(\beta, \tau^2, \lambda_1, \cdots, \lambda_n) \propto \pi(\tau^2) \prod_{i=1}^n \pi(\lambda_i)$. Here the $\tau^2$ is known as the global parameter and the $\lambda^2_i$ are known as the local parameters.  The Global-Local (GL) model also does away with the common variance assumption because the variance of a given random effect $u_i$ is a product of the global and local parameters $\lambda_i^2 \cdot \tau^2$ which allows for heterogeneity.  An extension of the model above was introduce in Tang and Ghosh (2023) where 
\begin{align}
  \bb u \given \tau^2, \Lambda \sim N_n(\bb 0, \tau^2 \Lambda^{1/2}Q^{-1}\Lambda^{1/2} ), 
\end{align}
where $Q$ is the CAR precision matrix, $\Lambda^{1/2}$ is the matrix square root of $\Lambda$, and this is used with the prior $\pi( \rho, \beta, \tau^2, \lambda_1, \cdots, \lambda_n) \propto \pi(\rho) \pi(\tau^2) \prod_{i=1}^n \pi(\lambda_i) $. This allows for random effects that that are spatially dependent while the shrinkage parameters remain independent.  

\todo[inline, color=green!40]{ $\uparrow$  Section could be significantly shortened. }
$\hline$


We can see from FIGURE xX  that using the Datta-Mandal model, unaccounted spatial dependence can appear in two ways. One way is through the random effects $\bb u = \bb \delta \odot \bb v $ and the other is through posterior inclusion probabilities $\bb{\tilde p}$.  Spatial dependence in $\bb{\tilde p}$ means that if a random effect is included in one area then it is likely needed in a neighboring area while dependence in $\bb \delta \odot \bb v$ means that the random effects that are selected are spatially correlated. This motivated the following extension. 
